Pareto-Secure Machine Learning (PSML): Fingerprinting and Securing Inference Serving Systems

Model-serving systems have become increasingly popular, especially in real-time web applications. In such systems, users send queries to the server and specify the desired performance metrics (e.g., desired accuracy, latency). The server maintains a set of models (model zoo) in the back-end and serves the queries based on the specified metrics. This paper examines the security, specifically robustness against model extraction attacks, of such systems. Existing black-box attacks assume a single model can be repeatedly selected for serving inference requests. Modern inference serving systems break this assumption. Thus, they cannot be directly applied to extract a victim model, as models are hidden behind a layer of abstraction exposed by the serving system. An attacker can no longer identify which model she is interacting with. To this end, we first propose a query-efficient fingerprinting algorithm to enable the attacker to trigger any desired model consistently. We show that by using our fingerprinting algorithm, model extraction can have fidelity and accuracy scores within $1\%$ of the scores obtained when attacking a single, explicitly specified model, as well as up to $14.6\%$ gain in accuracy and up to $7.7\%$ gain in fidelity compared to the naive attack. Second, we counter the proposed attack with a noise-based defense mechanism that thwarts fingerprinting by adding noise to the specified performance metrics. The proposed defense strategy reduces the attack's accuracy and fidelity by up to $9.8\%$ and $4.8\%$, respectively (on medium-sized model extraction). Third, we show that the proposed defense induces a fundamental trade-off between the level of protection and system goodput, achieving configurable and significant victim model extraction protection while maintaining acceptable goodput ($>80\%$). We implement the proposed defense in a real system with plans to open source.

==> conclusion-AT.tex <==
\section{Conclusion}
We make an observation that model extraction attacks make outdated assumptions that the victim model can be explicitly specified and directly queried. This is no longer true in state-of-the-art ML model serving systems. A novel, query-efficient fingerprinting algorithm re-enables model extraction, bridging the performance gap lost to implicit and dynamic model switching. Indeed, the proposed attack comes close to the single model serving setting, which \sys absorbs as a special case.
The proposed attack is shown effective over a wide range of model latencies, successfully extracting large, medium, and small-sized models from the zoo hidden behind the layer of model-less abstraction.
We defend against the proposed attack with a novel defense mechanism based on perturbation of (latency, accuracy) constraint specification with $\epsilon-$controlled noise. Doing so helps expose a practical tradeoff space between the system's level of defense and its performance, captured by its goodput. We show that robust levels of defense can be achieved with acceptable loss in system goodput.
The proposed attack and defense mechanisms are instantiated in a real system, with plans to open source to the community.
With a growing number of proprietary models served via implicit model selection in state-of-the-art inference systems, we make the first step towards better understanding the security implications of such systems with respect to Intellectual Property theft through model extraction.

